Benchmarking PhD-Level Coding in 3D Geometric Computer Vision

AI-assisted coding has rapidly reshaped software practice and research workflows, yet today's models still struggle to produce correct code for complex 3D geometric vision. If models could reliably write such code, the research of our community would change substantially. To measure progress toward that goal, we introduce GeoCodeBench, a PhD-level benchmark that evaluates coding for 3D vision. Each problem is a fill-in-the-function implementation task curated from representative papers at recent venues: we first let a tool propose candidate functions from official repositories, then perform careful human screening to select core 3D geometric components. For every target, we generate diverse, edge-case unit tests, enabling fully automatic, reproducible scoring. We evaluate eight representative open- and closed-source models to reflect the current ecosystem. The best model, GPT-5, attains only 36.6% pass rate, revealing a large gap between current capabilities and dependable 3D scientific coding. GeoCodeBench organizes tasks into a two-level hierarchy: General 3D capability (geometric transformations and mechanics/optics formulation) and Research capability (novel algorithm implementation and geometric logic routing). Scores are positively correlated across these axes, but research-oriented tasks are markedly harder. Context ablations further show that "more paper text" is not always better: cutting off at the Method section statistically outperforms full-paper inputs, highlighting unresolved challenges in long-context scientific comprehension. Together, these findings position GeoCodeBench as a rigorous testbed for advancing from generic coding to trustworthy 3D geometric vision coding.

==> sec/4_exp-old.tex <==
\section{Diagnosing LLMs on GeoCodeBench}

\label{sec:experiment}
In this section, we introduce our systematic framework for evaluating Large Language Models on the GeoCodeBench benchmark.



To comprehensively evaluate LLMs, we conducted zero-shot inference across both commercial and open-source models. Flag-ship Model.
GPT-5, Gemini-2.5-Pro, Kimi-K2, Doubao-seed-1.6, DeepSeek-R1, Claude-Sonnet-4.5, Llama-3.1-405B, Qwen3-Coder-480B.

\begin{tcolorbox}[
    colback=pink!10,       % 背景颜色（浅粉）
    colframe=red!70!black, % 边框颜色（深红）
    coltitle=white,        % 标题文字颜色
    fonttitle=\bfseries,   % 标题字体加粗
    title=Questions,       % 标题内容
    arc=6pt,               % 圆角大小
    boxrule=1pt,           % 边框线条粗细
    left=4pt, right=4pt, top=4pt, bottom=4pt, % 内边距
]
\begin{itemize}[leftmargin=1em]
    \item \textbf{Q1:} What are the baseline xxx(Main result)
    \item \textbf{Q2:} Can the  xxx(Ablation)
    \item \textbf{Q3:} How can we xxxx (Improvement)
\end{itemize}
\end{tcolorbox}

\subsection{Main results}
\input{tabs/TabMain}
\paragraph{Experimental Setup.} xxx

\paragraph{Key Observations.} 

By task type, all models perform better on general 3D-knowledge questions than on paper-reading questions. Within the general 3D category, LLMs achieve higher accuracy on problems involving coordinate and view transformations than on those centered on other mathematical formulas. For paper-reading questions, models do better on functionality-oriented tasks than on implementing core algorithmic ideas.

By model, closed-source systems consistently outperform open-source ones, with Gemini 2.5 Pro attaining the highest accuracy (30.7\%) and Kimi K2 the lowest (17.5\%). Even at comparable overall accuracy levels, models exhibit different strengths: for example, Doubao tends to excel on functionality-focused code, whereas Claude is stronger on coordinate-transformation tasks.

\paragraph{Insights.} 
(1).Because large language models (LLMs) are, at their core, statistical learners, they tend to produce common implementation patterns when confronted with novel algorithmic contributions in papers, rather than adhering to the paper-specific design intended by the authors.
(2).For questions that assess 3D knowledge, we observe that LLMs can generally reason correctly about the mathematical and physical formulas appearing in the paper. The dominant failure mode arises during \emph{implementation}, not reasoning.
(3).For paper-algorithm implementation tasks, LLMs can use function names and templates to accurately locate the relevant sections of the paper. Success correlates with how explicitly the paper specifies the method: when equations and procedures are highlighted in detail, accuracy is higher; when key steps are underspecified, code correctness drops, indicating limited capacity for filling implementation by reasoning.
(4).In terms of code-generation style, models prefer writing raw Python from scratch and rarely leverage third-party libraries or existing codebase utilities. They also exhibit a ``greedy'' tendency: optimizing for immediate task completion while paying less attention to code style, consistency with repository conventions, or broader architectural constraints.




\subsection{Ablation: Paper Input length}


\subsection{Failure Case Analysis}

\subsection{Case Study}

% Paste this directly into your paper body.
\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figs/3DGS Benchmark_04.png}
  \caption{Case 1. Some LLMs fail to understand the paper and overlook the cross reprojection between the Yin–Yang grids. we are polishing the figure, it is not the final version due to lack of beauty.
}
  \label{fig:1}
\end{figure*}

\paragraph*{Case 1}
This case comes from OmniSplat to evaluate whether a large language model (LLM) can read a paper, recover the authors’ algorithmic intent, which warps features bidirectionally between the Yin and Yang charts so that evidence is shared across gridst. In contrast, an LLM-generated implementation that omits cross-grid interactions amplifies missing evidence near the poles and chart boundaries, degrading both depth estimation and the regression of 3D Gaussian Splatting (3DGS) parameters. Empirically, contemporary LLMs can reproduce standard depth-estimation components—such as cost-volume construction and cross-view reprojection. However, the model misinterpreted the word “cross” in the function name as cross-attention across views, rather than cross-grid warping that exchanges information between Yin and Yang charts.. This case suggests that LLMs struggle to explore and implement new variants: they imitate cost-volume construction and cross-view projection well, but are weak at applying them flexibly. 


\medskip


\paragraph*{Case 2}
This function implements the Cook--Torrance microfacet \emph{specular} BRDF\todo{cite} using the GGX (Trowbridge--Reitz)\todo{cite} normal distribution \(D\), the Smith \emph{correlated} masking–shadowing term \(G\), and the Schlick Fresnel approximation \(F\). The formulation is widely used in physically based rendering (PBR)\todo{cite}. We use this function to assess whether large language models (LLMs) can recall commonly used computer-vision/graphics formulas \emph{and} translate them into correct code. According to the reasoning traces, LLMs generally remember the formulas; the primary issues arise during implementation.

\item \textbf{Roughness misparameterization.}
  Several models (e.g., GPT, Gemini, Kimi) pass \(\alpha\) where \(\alpha^2\) is required, which distorts the GGX highlight width and energy and thus the perceived roughness. In our setup, the helper functions \texttt{bsdf\_ndf\_ggx}, \texttt{bsdf\_lambda\_ggx}, and \texttt{bsdf\_masking\_smith\_ggx\_correlated} are specified to take \(\alpha^2\) as input, whereas the main entry \texttt{bsdf\_pbr\_specular} receives \(\alpha\).
  We infer that LLMs were misled into assuming the main function also expects \(\alpha^2\).
  In practice, LLMs must reconcile heterogeneous interface contracts scattered across a repository, but they are prone to errors driven by statistical priors instead of precise contract reasoning.

\item \textbf{Misuse of the specular color}.}
  In doubao, \texttt{col} is used as \(F_0\) (inside the Fresnel term) and then multiplied again in the final BRDF, effectively double-counting the specular color and producing overly bright materials. This likely stems from conflating two different formula conventions.\todo{cite}
  In qwen3, \texttt{col} is treated as an external scale while \(F_0\) is fixed to \(0.04\) (a dielectric constant), which prevents representing colored metallic Fresnel at normal incidence.
  These mistakes indicate a lack of \emph{contract comprehension}: the models fail to align parameter names with their physical semantics and to preserve that mapping consistently throughout the code.

We also observe syntactic, identifier errors. For example, in qwen3, the function \texttt{bsdf\_masking\_smith\_ggx\_correlated} declares parameters \texttt{cosThetaI} and \texttt{cosThetaO}, but the body references the undefined names \texttt{cosThetaV} and \texttt{cosThetaL}.












\medskip

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figs/3DGS Benchmark_06.png}
  \caption{Case 3. Some LLMs generate Gaussian points from triangular meshes that do not conform to the specifications of the paper. we are polishing the figure, it is not the final version due to lack of beauty.
}
  \label{fig:3}
\end{figure*}


\paragraph*{Case 3}

This case comes from GeoSplatting\cite{GeoGaussian} and implements the MGadapter\cite{GeoGaussian}, which madps geometric elements sampled from a triangular mesh (e.g., via barycentric/edge sampling)\todo{cite} to elliptical Gaussian splats suitable for 3D Gaussian Splatting---i.e., position, orientation, scales, color, opacity, etc. Conceptually, each splat should be a thin, anisotropic surfel: highly elongated within the local tangent plane and extremely thin along the normal. The core is to align the long axis with the geometric direction, derive the short axis adaptively from area, and enforce near-zero thickness along the normal.\todo{cite}
However, the LLM-produced implementation uses isotropic splats with non-negligible thickness, which violates the required geometry--Gaussian consistency and, in turn, degrades self-occlusion handling\todo{cite}, normal fidelity\todo{cite}, PBR light transport\todo{cite}, material decomposition\todo{cite}, and relighting quality\todo{cite}.

This function evaluates a model's ability to read the paper and implement the central algorithmic idea. Our experiments show that current LLMs have a solid grasp of common 3DGS geometric quantities. Nevertheless, they fail to internalize the MGadapter's special requirements from the paper and tend to produce a more generic, isotropic ellipsoid---reflecting the limitations of a statistical model. Because the MGadapter's specifics are not fully spelled out in the main text, a correct implementation requires not only reading and transcribing formulas but also understanding the algorithmic intent and flexibly applying geometric knowledge. This case therefore illustrates that, given limited details, LLMs still struggle to explore and select the most appropriate implementation.

==> tabs/TabAbility.tex <==

\begin{table}[t]
\tiny
\centering
\caption{\textbf{Model Capability Comparison}}
\label{tab:model-capability}
\renewcommand{\arraystretch}{1.2} % 行间距
\setlength{\tabcolsep}{6pt}      % 列间距
\newcolumntype{Y}{>{\centering\arraybackslash}X} % 定义居中可伸缩列

\begin{tabularx}{0.9\linewidth}{Y Y Y}  %
\toprule
\textbf{Model} & \textbf{General 3D Capability} & \textbf{Paper Specific Capability} \\ 
\midrule
Claude-Sonnet-4.5       & 33.2\%                         & 17.7\%                             \\
DeepSeek-R1             & 22.9\%                         & 8.0\%                              \\
Doubao-Seed-1.6         & 24.6\%                         & 19.4\%                             \\
Gemini-2.5-Pro          & 31.7\%                         & 20.8\%                             \\
GPT-5                   & \textbf{34.4\%}                & 18.0\%                             \\
Kimi-K2-Instruct        & 27.3\%                         & 24.7\%                             \\
Llama-3.1-405B-Instruct & 17.0\%                         & 10.7\%                             \\
Qwen3-Coder-480B        & 22.2\%                         & \textbf{24.8\%}                    \\
\bottomrule
\end{tabularx}
\end{table}

==> tabs/TabAllPapers.tex <==
% Switch to one-column mode for the longtable
\onecolumn

% Define column types for the paper table
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}

\begin{small}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}

\begin{longtable}{@{}L{0.60\textwidth}C{0.08\textwidth}C{0.10\textwidth}L{0.18\textwidth}@{}}
\caption{Papers Used in GeoCodeBench, Their Categories, Number of Questions, and Venues.}
\label{tab:geocode_papers}\\
\toprule
\textbf{Paper Name} & \textbf{Category} & \textbf{\# Questions} & \textbf{Conference} \\
\midrule
\endfirsthead

\toprule
\textbf{Paper Name} & \textbf{Category} & \textbf{\# Questions} & \textbf{Conference (Year)} \\
\midrule
\endhead

\bottomrule
\endfoot


UVGS: Reimagining Unstructured 3D Gaussian Splatting using UV Mapping~\cite{rai2025uvgs}
  & SpV & 2 & CVPR 2025 \\

3DGUT: Enabling Distorted Cameras and Secondary Rays in Gaussian Splatting~\cite{wu20253dgut}
  & Cam & 3 & CVPR 2025 \\

OmniSplat: Taming Feed-Forward 3D Gaussian Splatting for Omnidirectional Images with Editable Capabilities~\cite{lee2025omnisplat}
  & 360 & 3 & CVPR 2025 \\

IRGS: Inter-Reflective Gaussian Splatting with 2D Gaussian Ray Tracing~\cite{gu2025irgs}
  & IR  & 3 & CVPR 2025 \\

Splatter-360: Generalizable 360$^\circ$ Gaussian Splatting for Wide-baseline Panoramic Images~\cite{chen2025splatter}
  & 360 & 3 & CVPR 2025 \\

GaussianSpa: An ``Optimizing-Sparsifying'' Simplification Framework for Compact and High-Quality 3D Gaussian Splatting~\cite{zhang2025gaussianspa}
  & Eff & 2 & CVPR 2025 \\

IncEventGS: Pose-Free Gaussian Splatting from a Single Event Camera~\cite{huang2025inceventgs}
  & Dyn & 4 & CVPR 2025 \\

Improving Gaussian Splatting with Localized Points Management~\cite{yang2025improving}
  & Eff & 2 & CVPR 2025 \\

DOF-GS: Adjustable Depth-of-Field 3D Gaussian Splatting for Post-Capture Refocusing, Defocus Rendering and Blur Removal~\cite{wang2025dof}
  & Cam & 3 & CVPR 2025 \\

4D Gaussian Splatting SLAM~\cite{li20254d}
  & Dyn & 3 & ICCV 2025 \\

Hardware-Rasterized Ray-Based Gaussian Splatting~\cite{bulo2025hardware}
  & Eff & 3 & CVPR 2025 \\

CoMoGaussian: Continuous Motion-Aware Gaussian Splatting from Motion-Blurred Images~\cite{lee2025comogaussian}
  & Cam & 3 & ICCV 2025 \\

Curve-Aware Gaussian Splatting for 3D Parametric Curve Reconstruction~\cite{gao2025curve}
  & Geo & 3 & ICCV 2025 \\

Gaussian Splatting with Discretized SDF for Relightable Assets~\cite{zhu2025gaussian}
  & IR  & 1 & ICCV 2025 \\

Self-Ensembling Gaussian Splatting for Few-Shot Novel View Synthesis~\cite{zhao2025self}
  & SpV & 1 & ICCV 2025 \\

Splat-LOAM: Gaussian Splatting LiDAR Odometry and Mapping~\cite{giacomini2025splat}
  & Dyn & 2 & ICCV 2025 \\

Instant GaussianImage: A Generalizable and Self-Adaptive Image Representation via 2D Gaussian Splatting~\cite{zeng2025instant}
  & Eff & 2 & ICCV 2025 \\

MGSR: 2D/3D Mutual-boosted Gaussian Splatting for High-fidelity Surface Reconstruction under Various Light Conditions~\cite{zhou2025mgsr}
  & IR  & 3 & ICCV 2025 \\

DeGauss: Dynamic-Static Decomposition with Gaussian Splatting for Distractor-free 3D Reconstruction~\cite{wang2025degauss}
  & Dyn & 2 & ICCV 2025 \\

GeoSplatting: Towards Geometry Guided Gaussian Splatting for Physically-based Inverse Rendering~\cite{ye2025geosplatting}
  & IR  & 2 & ICCV 2025 \\

Toward Real-world BEV Perception: Depth Uncertainty Estimation via Gaussian Splatting~\cite{lu2025toward}
  & Geo & 5 & CVPR 2025 \\

PanSplat: 4K Panorama Synthesis with Feed-Forward Gaussian Splatting~\cite{zhang2025pansplat}
  & 360 & 4 & CVPR 2025 \\

RegGS: Unposed Sparse Views Gaussian Splatting with 3DGS Registration~\cite{cheng2025reggs}
  & SpV & 3 & ICCV 2025 \\

DashGaussian: Optimizing 3D Gaussian Splatting in 200 Seconds~\cite{chen2025dashgaussian}
  & Eff & 3 & CVPR 2025 \\

Taming Video Diffusion Prior with Scene-Grounding Guidance for 3D Gaussian Splatting from Sparse Inputs~\cite{zhong2025taming}
  & SpV & 4 & CVPR 2025 \\

Self-Calibrating Gaussian Splatting for Large Field of View Reconstruction~\cite{deng2025self}
  & Cam & 4 & ICCV 2025 \\

LUDVIG: Learning-Free Uplifting of 2D Visual Features to Gaussian Splatting Scenes~\cite{marrie2025ludvig}
  & SpV & 1 & ICCV 2025 \\

PolGS: Polarimetric Gaussian Splatting for Fast Reflective Surface Reconstruction~\cite{han2025polgs}
  & Geo & 4 & ICCV 2025 \\

FlexGS: Train Once, Deploy Everywhere with Many-in-One Flexible 3D Gaussian Splatting~\cite{liu2025flexgs}
  & Eff & 1 & CVPR 2025 \\

MonoSplat: Generalizable 3D Gaussian Splatting from Monocular Depth Foundation Models~\cite{liu2025monosplat}
  & SpV & 1 & CVPR 2025 \\

GaussianBlock: Building Part-Aware Compositional and Editable 3D Scene by Primitives and Gaussians~\cite{jiang2024gaussianblock}
  & Geo & 4 & ICLR 2025 \\

HoGS: Unified Near and Far Object Reconstruction via Homogeneous Gaussian Splatting~\cite{liu2025hogs}
  & Cam & 1 & CVPR 2025 \\

Sparse2DGS: Geometry-Prioritized Gaussian Splatting for Surface Reconstruction from Sparse Views~\cite{wu2025sparse2dgs}
  & SpV & 4 & CVPR 2025 \\

TetSphere Splatting: Representing High-Quality Geometry with Lagrangian Volumetric Meshes~\cite{guo2024tetsphere}
  & Geo & 3 & ICLR 2025 \\

Reflective Gaussian Splatting~\cite{yao2024reflective}
  & IR  & 5 & ICLR 2025 \\

Fast Feedforward 3D Gaussian Splatting Compression~\cite{chen2024fast}
  & Eff & 2 & ICLR 2025 \\

SurFhead: Affine Rig Blending for Geometrically Accurate 2D Gaussian Surfel Head Avatars~\cite{lee2024surfhead}
  & Geo & 4 & ICLR 2025 \\
  
EMD: Explicit Motion Modeling for High-Quality Street Gaussian Splatting~\cite{wei2025emd}
  & Dyn & 3 & ICCV 2025 \\


\end{longtable}

\vspace{0.5em}
\noindent\textbf{Category legend:}
IR = Inverse rendering / illumination;
Cam = Camera / optics / projection;
360 = 360$^\circ$/omnidirectional;
SpV = Sparse-view / generalization / priors;
Dyn = Dynamic scenes / SLAM / non-RGB;
Eff = Efficiency / compression / optimization;
Geo = Specialized geometry / editing / applications.

\end{small}

% Switch back to two-column mode
\twocolumn

==> tabs/TabFull.tex <==
\begin{table*}[]
\caption{\textbf{Tab Full (for reference)}}
\begin{tabular}{cccccc}
\hline
\textbf{Model}        & \textbf{Score} & \textbf{\begin{tabular}[c]{@{}c@{}}Geometric\\  Transformations\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Mathematical\\  Formulation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Algorithm\\  Implementation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Module\\  Integration\end{tabular}} \\ \hline
llm\_claude-full      & 27.2\%         & 41.9\%                                                                        & 28.5\%                                                                       & 17.2\%                                                                       & 20.0\%                                                                 \\
llm\_claude-method    & 28.3\%         & 40.9\%                                                                        & 23.5\%                                                                       & 23.5\%                                                                       & 38.3\%                                                                 \\
llm\_claude-nopaper   & 28.4\%         & 45.7\%                                                                        & 26.0\%                                                                       & 21.3\%                                                                       & 21.7\%                                                                 \\ \hline
llm\_deepseek-full    & 17.1\%         & 36.7\%                                                                        & 15.6\%                                                                       & 8.7\%                                                                        & 5.0\%                                                                  \\
llm\_deepseek-method  & 25.8\%         & 27.7\%                                                                        & 27.9\%                                                                       & 21.7\%                                                                       & 26.7\%                                                                 \\
llm\_deepseek-nopaper & 27.3\%         & 48.2\%                                                                        & 24.7\%                                                                       & 18.0\%                                                                       & 21.7\%                                                                 \\ \hline
llm\_doubao-full      & 22.6\%         & 41.1\%                                                                        & 16.0\%                                                                       & 19.3\%                                                                       & 20.0\%                                                                 \\
llm\_doubao-method    & 27.2\%         & 40.3\%                                                                        & 25.2\%                                                                       & 17.3\%                                                                       & 43.3\%                                                                 \\
llm\_doubao-nopaper   & 23.9\%         & 36.8\%                                                                        & 20.3\%                                                                       & 15.6\%                                                                       & 43.3\%                                                                 \\ \hline
llm\_gemini-full      & 27.4\%         & 44.0\%                                                                        & 25.2\%                                                                       & 17.2\%                                                                       & 36.7\%                                                                 \\
llm\_gemini-method    & 32.2\%         & 46.2\%                                                                        & 29.7\%                                                                       & 22.0\%                                                                       & 50.0\%                                                                 \\
llm\_gemini-nopaper   & 26.7\%         & 43.6\%                                                                        & 23.5\%                                                                       & 15.3\%                                                                       & 45.0\%                                                                 \\ \hline
llm\_gpt-full         & 28.0\%         & 35.1\%                                                                        & 34.0\%                                                                       & 17.2\%                                                                       & 21.7\%                                                                 \\
llm\_gpt-method       & 29.4\%         & 40.1\%                                                                        & 31.9\%                                                                       & 19.4\%                                                                       & 28.3\%                                                                 \\
llm\_gpt-nopaper      & 28.6\%         & 40.7\%                                                                        & 27.4\%                                                                       & 20.6\%                                                                       & 35.0\%                                                                 \\ \hline
llm\_kimi-full        & 26.3\%         & 38.8\%                                                                        & 21.2\%                                                                       & 25.4\%                                                                       & 21.7\%                                                                 \\
llm\_kimi-method      & 29.9\%         & 41.6\%                                                                        & 24.6\%                                                                       & 30.7\%                                                                       & 21.7\%                                                                 \\
llm\_kimi-nopaper     & 26.5\%         & 35.9\%                                                                        & 24.1\%                                                                       & 19.4\%                                                                       & 43.3\%                                                                 \\ \hline
llm\_llama-full       & 14.5\%         & 25.7\%                                                                        & 12.4\%                                                                       & 4.9\%                                                                        & 36.7\%                                                                 \\
llm\_llama-method     & 17.1\%         & 25.4\%                                                                        & 21.6\%                                                                       & 8.9\%                                                                        & 3.3\%                                                                  \\
llm\_llama-nopaper    & 15.0\%         & 25.4\%                                                                        & 20.9\%                                                                       & 3.3\%                                                                        & 3.3\%                                                                  \\ \hline
llm\_qwen-full        & 23.2\%         & 31.2\%                                                                        & 17.5\%                                                                       & 26.6\%                                                                       & 16.7\%                                                                 \\
llm\_qwen-method      & 25.3\%         & 36.9\%                                                                        & 27.8\%                                                                       & 15.4\%                                                                       & 21.7\%                                                                 \\
llm\_qwen-nopaper     & 24.4\%         & 36.9\%                                                                        & 21.6\%                                                                       & 16.9\%                                                                       & 36.7\%                                                                 \\ \hline
\end{tabular}
\end{table*}

==> tabs/TabMain_Old.tex <==
\begin{table*}[t]
\centering 
\small
\caption{\textbf{The Performance of Representative LLMs on GeoCodeBench.} Performance is assessed across four dimensions:  \textit{Geometric Transformations} (Geo. Trans.),  \textit{Mechanics/Optics Formulation} (Mech./Opt.), \textit{Novel Algorithm Implementation}(Algorithm), and \textit{Geometric Logic Routing}(Routing).}
\label{tab:main}
\renewcommand{\arraystretch}{1.05} % 行间距调节
% \setlength{\tabcolsep}{6pt}       % 列间距调节
\begin{tabularx}{\textwidth}{
    l|cc|c|
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
}
\toprule
 & {} 
 & {} 
 & 
 & \multicolumn{2}{c}{\textbf{General 3D Capability}} 
 & \multicolumn{2}{c}{\textbf{Research Capability}} \\
\multirow{-2}{*}{\textbf{Model}} 
 & \multirow{-2}{*}{{\textbf{Company}}} 
 & \multirow{-2}{*}{{\textbf{Type}}} 
 & \multirow{-2}{*}{\textbf{Overall}} 
 & \textbf{Geo. Trans.} 
 & \textbf{Mech./Opt.} 
 & \textbf{Algorithm} 
 & \textbf{Routing} \\ \midrule

% GPT-5 & OpenAI & closed-source  & \textbf{28.0\%} & 35.1\% & \textbf{34.0\%} & 17.2\% & 21.7\% \\
% Gemini-2.5-Pro & Google & closed-source  & 27.4\% & \textbf{44.0\%} & 25.2\% & 17.2\% & \textbf{36.7\%} \\
% Claude-Sonnet-4.5 & Anthropic & closed-source & 27.2\% & 41.9\% & 28.5\% & 17.2\% & 20.0\% \\
% Kimi-K2-Instruct & MoonshotAI & open-source & 26.3\% & 38.8\% & 21.2\% & 25.4\% & 21.7\% \\
% Qwen3-Coder-480B & Alibaba & open-source & 23.2\% & 31.2\% & 17.5\% & \textbf{26.6\%} & 16.7\% \\
% Doubao-Seed-1.6 & ByteDance & closed-source & 22.6\% & 41.1\% & 16.0\% & 19.3\% & 20.0\% \\
% DeepSeek-R1 & DeepSeek & open-source & 17.1\% & 36.7\% & 15.6\% & 8.7\% & 5.0\% \\
% Llama-3.1-405B-Instruct & Meta & open-source & 14.5\% & 25.7\% & 12.4\% & 4.9\% & \textbf{36.7\%} \\ \bottomrule



GPT-5 & OpenAI & closed-source  & \textbf{36.6\%} & 41.7\% & \textbf{43.7\%} & \textbf{29.1}\% & 28.9\% \\
Claude-Sonnet-4.5 & Anthropic & closed-source & 31.1\% & 38.3\% & 36.5\% & 19.7\% & \textbf{35.9\%} \\
Gemini-2.5-Pro & Google & closed-source  & 30.4\% & \textbf{41.9\%} & 27.6\% & 25.3\% & 29.1\%\\
Kimi-K2-Instruct & MoonshotAI & open-source & 30.4\% & 36.7\% & 33.1\% & 23.1\% & 31.4\% \\
Doubao-Seed-1.6 & ByteDance & closed-source & 26.9\% & 40.9\% & 21.0\% & 22.9\% & 25.2\% \\
Qwen3-Coder-480B & Alibaba & open-source & 23.5\% & 29.0\% & 17.7\% & 21.8\% & 33.2\% \\
DeepSeek-R1 & DeepSeek & open-source & 21.0\% & 33.9\% & 21.9\% & 12.4\% & 17.0\% \\
Llama-3.1-405B-Instruct & Meta & open-source & 14.3\% & 21.3\% & 13.2\% & 10.9\% & 12.7\% \\ \bottomrule

\end{tabularx}
\end{table*}



